Unveiling Backdoor Risks Brought by Foundation Models in Heterogeneous Federated Learning

The foundation models (FMs) have been used to generate synthetic public datasets for the heterogeneous federated learning (HFL) problem where each client uses a unique model architecture. However, the vulnerabilities of integrating FMs, especially against backdoor attacks, are not well-explored in the HFL contexts. In this paper, we introduce a novel backdoor attack mechanism for HFL that circumvents the need for client compromise or ongoing participation in the FL process. This method plants and transfers the backdoor through a generated synthetic public dataset, which could help evade existing backdoor defenses in FL by presenting normal client behaviors. Empirical experiments across different HFL configurations and benchmark datasets demonstrate the effectiveness of our attack compared to traditional client-based attacks. Our findings reveal significant security risks in developing robust FM-assisted HFL systems. This research contributes to enhancing the safety and integrity of FL systems, highlighting the need for advanced security measures in the era of FMs.

==> section/data.tex <==
\section{Data}
\textcolor{blue}{done}
\subsection{Dataset Overview}
The selected data is from the health insurance claims collected by IQVIA \footnote{\url{https://www.iqvia.com/}}. The EHR data includes patients' age, gender, zipcode, diagnosis code within each visit, the vaccine brand, and a binary label of the side effects. In this extracted dataset, there are 6526 patients with COVID-19 vaccinated. 1097 of them have side effects who are labeled as 1 and 5429 of them have no side effects who are labeled as 0 on the record. The unbalanced label ratio is around 5:1 (negative label : positive label). The vaccine brands are Moderna, Pfizer-BioNTech, and Janssen. The number of patients with the brands of vaccine are 3355, 2159, and 1012 respectively.  The basic statistic of the dataset is shown in Table \ref{tab:iqvia_stat}. 

\begin{table}[htbp]
\caption{Data statistics of the selected IQVIA dataset } 
% \vspace{-0.1in}
\label{tab:iqvia_stat}
\centering 
\begin{tabular}{lclc}
\toprule
Patient Count                 & 6526 & Moderna & 3355 \\
Positive Patient Count     & 1097 & Pfizer-BioNTech & 2159 \\
Negative Patient Count         & 5429& Janssen & 1012  \\
Male&1761& ICD Code Count & 803\\
Female& 4765&State Count   &29\\
\bottomrule
\end{tabular} 
\end{table}

The dataset also provides geography information via the zipcodes. Based on the zipcode information, patients are from 29 states. However, the data distribution of states is extremely unequal. There are 1409 patients from CA, while where are only 35 patients in MD, OK, and UT on the record. We highlight the 10 states with more than 200 patients with green and the visualize the data geological information in Figure \ref{fig:map}.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\textwidth]{figure/map.pdf}
\caption{Patient geographical distribution across states. The large states (green) are the states with the total data larger than 200 and the normal states (normal) are the states with the total data less than 200.}
\label{fig:map}
\end{figure}




% \begin{table}[htbp]
% \caption{Data statistics of extracted IQVIA dataset } 
% \label{tab:iqvia_statistics}
% \centering 
% \begin{tabular}{lclc}
% \toprule
% Patient Count                 & 6526    &  vaccine type & 3\\
% - & - & Moderna & 3355 \\
% - & - & Pfizer-BioNTech & 2159 \\
% - & - & Janssen & 1012 \\
% Positive Patient Count     & 1097 & Training Patient Count &  5006     \\
% Negative Patient Count         & 5429 &  Training Positive Patient Count &  879  \\
% Male&1761& Training Negative Patient Count &  4127           \\
% Female& 4765& Test Patient Count & 1520\\
% ICD Code Count & 803 &Test Positive Patient Count &     218     \\
% State Count   &29& Test Negative Patient Count & 1302 \\
% \bottomrule
% \end{tabular} 
% \end{table}
\subsection{Training and Test Data Construction}\label{train_test}
As it is not a benchmark dataset with well-established training and test split, we will introduce how we create our training and test datasets. To keep as much as the original information of the whole dataset, we split the data based on the geological information and label distribution. To preserve the data privacy, we treat each state as an individual client in our framework. For each state, we rawly sample 80\% data for training and 20\% data for test for positive label and negative label accordingly. 

After that, We keep the training data of each state locally for each client to train local models separately. We merge the test data from each state into a large test dataset for the global model test use. In this way, we preserve the data privacy for each state without sharing patient's data for model training. On the other hand, we construct the training and test data with maintaining the similar label distribution geologically as much as we can. The basic statistic of the training and test data is shown in Table \ref{tab:train_test_stat}. The label ratio of training and test data from different states is visualized in Figure.

\begin{table}[htbp]
\caption{Data statistics of extracted IQVIA dataset } 
\label{tab:iqvia_statistics}
\centering 
\begin{tabular}{lclc}
\toprule
Training Patient Count &  5006  & Test Patient Count & 1520   \\
Training Positive Patient Count & 879 &Test Positive Patient Count &     218 \\
Training Negative Patient Count &  4127    & Test Negative Patient Count & 1302        \\
\bottomrule
\end{tabular}
\label{tab:train_test_stat}
\end{table}


\begin{figure}[htbp]
\centering
\includegraphics[width=1\textwidth]{figure/train_test_state.pdf}
\caption{Training and test data label ratio for each state}
\label{fig:train_test_data}
\end{figure}
\subsection{Data Challenges}
Compared with traditional benchmark data, we have several challenges raised by our data itself, which generally represent common features of real-world data.
\begin{itemize}
    \item \textbf{Unbalanced Label} For this vaccine-related dataset, the positive label over the negative label is around 1 over 5, which is unbalanced labeled dataset;
    \item \textbf{Unbalanced Data Size} Different states are treated as different clients to keep its own data private. However, as shown in Figure \ref{fig:map}, the data size varies from 1409 to 35. It is challenging to leverage such an unbalanced series of data to train an identical backbone;
    
    \item \textbf{Limited Data} There are 19 states where the data is less than 200 patients, which raises a small data challenge. When we do the global model aggregation, how to treat the models trained from the clients with small data appropriately would be another challenge.
    \item \textbf{Data Type} Most research works of federated learning focus on image data task. Our data includes categorical data, numerical data, and time-series EHR data. Besides that, to our best knowledge, this is the first work to predict COVID-19 vaccine side effects based on the fusion of different types of patients' data considering the geological information.
    
\end{itemize}

==> section/data_new.tex <==
\section{COVID-19 Vaccine EHR Data}\label{sec:data}
\subsection{Dataset Overview}
We extracted the EHR data from the health insurance claims database of IQVIA. 
Similar to other types of data~\cite{DBLP:conf/sdm/ZhouYH17,DBLP:conf/icdm/ZhouH17}, EHR data are \textbf{heterogeneous}, which include patients' age, gender, zip code, diagnosis codes within each visit, the vaccine brand, and a binary label of the side effects. In this extracted dataset, there are 6,526 patients with COVID-19 vaccinated. 1,097 of them have side effects who are labeled as 1, and 5429 of them have no side effects who are labeled as 0 on the record. The \textbf{imbalanced} label ratio is around 1:5 (\# of positive labels : \# of negative labels). The vaccine brands include Moderna, Pfizer-BioNTech, and Johnson \& Johnson's Janssen. The number of patients with the brands of vaccines is 3,355, 2,159, and 1,012, respectively. The basic statistic of the dataset is shown in Table \ref{tab:iqvia_stat}. 


% The selected data is from the health insurance claims collected by IQVIA \footnote{\url{https://www.iqvia.com/}}. The EHR data includes patients' age, gender, zipcode, diagnosis code within each visit, the vaccine brand, and a binary label of the side effects. In this extracted dataset, there are 6526 patients with COVID-19 vaccinated. 1097 of them have side effects who are labeled as 1 and 5429 of them have no side effects who are labeled as 0 on the record. The unbalanced label ratio is around 5:1 (negative label : positive label). The vaccine brands are Moderna, Pfizer-BioNTech, and Janssen. The number of patients with the brands of vaccine are 3355, 2159, and 1012 respectively.  The basic statistic of the dataset is shown in Table \ref{tab:iqvia_stat}. 

\begin{table}[!t]
\caption{Data statistics of the extracted EHR dataset. } 
% \vspace{-0.1in}
\label{tab:iqvia_stat}
\centering 
\begin{tabular}{lcclc}
\toprule
Patient Count                 & 6,526 &\;& Moderna & 3,355 \\
Positive Patient Count     & 1,097 && Pfizer-BioNTech & 2,159 \\
Negative Patient Count         & 5,429&& Janssen & 1,012  \\
Male&1,761&& ICD Code Count & 803\\
Female& 4,765&&State Count   &29\\
\bottomrule
\end{tabular} 
\end{table}
\begin{figure}[!t]
\centering
\includegraphics[width=0.7\textwidth]{figure/map_updated.pdf}
\caption{Patient geographical distribution across states. The states marked in green color are the ones with the total number of data larger than 200.}
\label{fig:map}
\vspace{-0.15in}
\end{figure}

The dataset also provides geographic visualization via the zip codes. Based on the zip code information, patients are from 29 states. However, the \textbf{data distribution of states} is extremely \textbf{unequal}. There are 1,409 patients from CA, while there are only 35 patients in MD, OK, and UT in the dataset. We highlight the 10 states with more than 200 patients in green and visualize the data with geological information in Figure \ref{fig:map}. There are 19 states where the data is less than 200 patients, which raises a \textbf{small data challenge}. When we do global model aggregation for federated learning, how we treat the models trained by the small clients appropriately will be a new practical challenge for the COVID-19 vaccine side effect prediction task.





% \begin{table}[htbp]
% \caption{Data statistics of extracted IQVIA dataset } 
% \label{tab:iqvia_statistics}
% \centering 
% \begin{tabular}{lclc}
% \toprule
% Patient Count                 & 6526    &  vaccine type & 3\\
% - & - & Moderna & 3355 \\
% - & - & Pfizer-BioNTech & 2159 \\
% - & - & Janssen & 1012 \\
% Positive Patient Count     & 1097 & Training Patient Count &  5006     \\
% Negative Patient Count         & 5429 &  Training Positive Patient Count &  879  \\
% Male&1761& Training Negative Patient Count &  4127           \\
% Female& 4765& Test Patient Count & 1520\\
% ICD Code Count & 803 &Test Positive Patient Count &     218     \\
% State Count   &29& Test Negative Patient Count & 1302 \\
% \bottomrule
% \end{tabular} 
% \end{table}
\subsection{Training and Test Data Construction}\label{train_test}
As it is not a benchmark dataset with a well-established training and test split, we will introduce how we create our training and test datasets. To keep as much of the original information as possible, we split the data based on the geological information and label distribution. To preserve data privacy, we treat each state as an individual client in our framework. For each state, we randomly sample 80\% data for training and 20\% data for testing on positive labels and negative labels accordingly.

After that, we keep the training data of each state locally for each client to train the local model. We merge the test data from each state into a large dataset for testing the performance of the global model. In such a way, we preserve the data privacy for each state without sharing patients' data for model training. On the other hand, we construct the training and test data while preserving as much of the geologically similar label distribution as possible.The basic statistics of the training and test data are shown in Table \ref{tab:train_test_stat}. The label ratio of training and test data from different states is visualized in Figure~\ref{fig:train_test_data}.

% \begin{table}[!t]
% \caption{Training and testing data statistics.} 
% \label{tab:iqvia_statistics}
% \centering 
% \begin{tabular}{lcclc}
% \toprule
% Training Patient Count &  5,006  &\;& Testing Patient Count & 1,520   \\
% Training Positive Patient Count & 879 &\;&Testing Positive Patient Count &     218 \\
% Training Negative Patient Count &  4,127    &\;& Testing Negative Patient Count & 1,302        \\
% \bottomrule
% \end{tabular}
% \label{tab:train_test_stat}
% \end{table}

\begin{table}[!t]
\caption{Training and testing data statistics.} 
\label{tab:iqvia_statistics}
\centering 
\begin{tabular}{lc|lc}
\toprule
\multicolumn{2}{c|}{Training}  &  \multicolumn{2}{c}{Testing} \\
\midrule
\# Patient  &  5,006  & \# Patient  & 1,520   \\
\#  Positive Patient  & 879 &\#  Positive Patient  &     218 \\
\#  Negative Patient  &  4,127   & \#  Negative Patient  & 1,302        \\
\bottomrule
\end{tabular}
\label{tab:train_test_stat}
\end{table}


\begin{figure}[!t]
\centering
\includegraphics[width=1\textwidth]{figure/train_test_state.pdf}
\caption{Training and test data label ratio for each state.}
\label{fig:train_test_data}
\end{figure}
% \subsection{Data Challenges}
% Compared with traditional benchmark data, we have several challenges raised by our dataset itself, which generally represent common features of real-world EHR datasets.
% \begin{itemize}
%     \item \textbf{Unbalanced Label} For this vaccine-related dataset, the positive label over the negative label is around 1 over 5, which is unbalanced labeled dataset;
%     \item \textbf{Unbalanced Data Size} Different states are treated as different clients to keep its own data private. However, as shown in Figure \ref{fig:map}, the data size varies from 1409 to 35. It is challenging to leverage such an unbalanced series of data to train an identical backbone;
    
%     \item \textbf{Limited Data} There are 19 states where the data is less than 200 patients, which raises a small data challenge. When we do the global model aggregation, how to treat the models trained from the clients with small data appropriately would be another challenge.
%     \item \textbf{Data Type} Most research works of federated learning focus on image data task. Our data includes categorical data, numerical data, and time-series EHR data. Besides that, to our best knowledge, this is the first work to predict COVID-19 vaccine side effects based on the fusion of different types of patients' data considering the geological information.
    
% \end{itemize}

==> section/task_notation.tex <==
\section{Task \& Notations}
In this paper, we focus on personalized federated learning by constructing clusters and graphs dynamically for active clients in each iteration. To maximize the local model performance, we distribute the models precisely back to the clients as their model initialization. Assume that there are $K$ clients, and each client $k$ holds data denoted as $\mathcal{D}_k = \{x_i^k\}_{i= 1}^{N_k}$, where $N_k$ is the number of data stored in the $k$-th client. At time $t$, the local model parameters trained with $\mathcal{D}_k$ are denoted as $\mathbf{w}_k$. After $B$ clients' model parameters are uploaded to the server, they are grouped into $Q$ clusters and the model belonging to cluster $q$ is denoted as $\mathbf{w}_k^q$. The center of cluster $q$ is equipped with $\mathbf{w}_s^q$, which is also formulated as a node in the graph as well. $\mathbf{p}$ represents the times that we conduct model parameter propagation across the graph. After that, we get an updated model parameter $\mathbf{w}_s^{q+}$ for the node $q$. More notations can be found in the Table \ref{tab:notation}.


\begin{table}[!tbp]
\centering
\caption{Notation Table.}
% \resizebox{0.8\textwidth}{!}{
\label{tb:natation}
\begin{tabular}{cl}
\toprule
Symbol  & Definition and description \\
          \midrule
$\mathcal{D}_k$ & the set of labeled data on the $k$-th client\\
% $\hat{\mathcal{D}}_k^{+}$ & the set of high-quality pseudo labeled data at client $k$\\
K & the number of clients\\
$\gamma$ & active ratio of clients \\
B & the number of active/selected clients\\
Q & the number of clusters\\
$\mathbf{w}_k$ & the $k$-th client's local model parameters\\
$\mathbf{w}_k^q$ & the $k$-th client's local model parameters in group $q$\\
$\mathbf{w}_s^q$ & model parameters of cluster center $q$\\
$\mathcal{W}_s^q$ & the cluster center model sets\\
$\mathbf{w}_s^{q+}$ & updated model parameters of cluster center $q$\\
$\mathbf{P}$ & the number of knowledge propagation times across the graph \\
$\mathcal{G}_t$ & the constructed graph at communication round t\\
\bottomrule
\end{tabular}
% }
\label{tab:notation}
\end{table}
